Learning to Solve Complex Problems via Dataset Decomposition

Curriculum learning is a class of training strategies that organizes the data being exposed to a model by difficulty, gradually from simpler to more complex examples. This research explores a reverse curriculum generation approach that recursively decomposes complex datasets into simpler, more learnable components. We propose a teacher-student framework where the teacher is equipped with the ability to reason step-by-step, which is used to recursively generate easier versions of examples, enabling the student model to progressively master difficult tasks. We propose a novel scoring system to measure data difficulty based on its structural complexity and conceptual depth, allowing curriculum construction over decomposed data. Experiments on math datasets (MATH and AIME) and code generation datasets demonstrate that models trained with curricula generated by our approach exhibit superior performance compared to standard training on original datasets.

==> algorithm_with_bug.tex <==
% \makebox[\textwidth]{
% \centering
% \resizebox{0.85\textwidth}{!}{
% \begin{varwidth}{\textwidth}
\begin{algorithmic}
\SetAlgoLined
\DontPrintSemicolon
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwComment{Comment}{$\triangleright$}{}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{DecomposeExample}{DecomposeExample}
\caption{Recursive Dataset Decomposition}
%\caption{Pseudo Code for Recursive Dataset Decomposition}
\label{algo:decomposition}
\small
\BlankLine
\Input{Problem set $\mathcal{D}_\text{raw}$, teacher model $\mathcal{T}$, maximum decomposition depth $D$, maximum steps per layer $k$}
\Output{Decomposed dataset $\mathcal{D}_\text{curr}$}

\BlankLine

Initialize empty dataset $\mathcal{D}_\text{curr} = \{\}$\;
\BlankLine
\Fn{\DecomposeExample{$q, cot, a, d, \mathcal{D}_{curr}$}}{
Split $cot$ into steps $\{s_1, \dots, s_k\}$ using $\mathcal{T}$\;
\BlankLine
\For{$i = 1$ \KwTo $k$}{
    Generate concept tag $t_i$ for step $s_i$ using $\mathcal{T}$\;
    \BlankLine
    \For{$\text{retry} = 1$ \KwTo MaxRetries}{
        Generate question $q_i$ from $(s_i, t_i) $ \;
        \BlankLine
        Generate step-by-step solution $cot_i$ and answer $a_i$ from $(q, s_i, t_i)$ using $\mathcal{T}$\;
        \BlankLine
        Verify $a_i$ via auto-solver and consistency check \emph{(see paper)} \;
        \BlankLine
        \If{verified}{
            Break\;
        }
    }
    \BlankLine
    $\mathcal{D}_{curr} = \mathcal{D}_{curr} \cup (q_i, cot_i, a_i, t_i, d)$\;
    \BlankLine
    \If{$d$ $<$ $D$}{
    \DecomposeExample{$q_i, cot_i, a_i, d + 1, \mathcal{D}_{curr}$}\; \emph{\# Recursive call}
    }
    }
}
\BlankLine
\ForEach{$(q, cot, a) \in \mathcal{D}_\text{raw}$}{
    \DecomposeExample{$q, cot, a, 0, \mathcal{D}_{curr}$}

    $\mathcal{D}_{curr} = \mathcal{D}_{curr} \cup (q, cot, a, -, \mathcal{D})$
}

%\State \Return{$\mathcal{D}_\text{curr}$}
}
\end{algorithm}



==> code_large_table.tex <==
\begin{table*}[t!]
\centering
\caption{Comparison of testing accuracy to LLMs on the HumanEval benchmark. \# data refers to the number of examples used for fine-tuning.}
\label{tab:perf_aime2025}
\begin{tabular}{lcc}
\toprule
\bf Model & \bf \makecell{\# data} & \bf \makecell{HumanEval pass@1} \\
%Flash Think.         &            &      \\
\midrule
\multicolumn{3}{c}{\textit{\textbf{Open-Weights Models}}} \\
\midrule
% Qwen2.5-1.5B~\citep{qwen2024qwen25technicalreport}        & N.A.       &  37.2 \\
Qwen2.5-3B~\citep{qwen2024qwen25technicalreport}             & N.A.       & 42.1 \\
Llama3-8B~\citep{dubey2024llama3herdmodels}          & N.A.       & 33.5 \\
Mistral-7B~\citep{jiang2024mixtral}        & N.A.       & 29.3 \\
Gemma2-9B~\citep{gemmateam2024gemma2improvingopen}           & N.A.       & 37.8\\
Llama-3-70B~\citep{dubey2024llama3herdmodels}          & N.A.       & 48.2 \\
Mixtral-8x22B~\citep{jiang2024mixtral}        & N.A.       & 46.3 \\
% \midrule
% Gemma2-9B-Instruct~\citep{gemmateam2024gemma2improvingopen}      & N.A.       & 68.9 \\
% Llama3.1-8B-Instruct~\citep{dubey2024llama3herdmodels}  & N.A.       & 72.6 \\
% \midrule
% Qwen2.5-72B-Instruct~\citep{qwen2024qwen25technicalreport}  & N.A.      & 86.6 \\
\midrule
\multicolumn{3}{c}{\textit{\textbf{Close-Source Models}}} \\
\midrule
GPT-4~\citep{openai2023gpt4}               & N.A.    & 67.0 \\
\midrule
\multicolumn{3}{c}{\textit{\textbf{Qwen2.5-1.5B-Instruct SFT on Codeforces-CoTs}}} \\
\midrule
Base                 & N.A.   & $34.15 \pm 3.71$ \\
SFT                  & xxx      & $35.37 \pm 3.74$ \\
%SFT-MetaMATH-AnsAug(Answer Augmentation) & 60& & TODO \\
%SFT-MetaMATH-Rephrasing & 60& & TODO \\
%SFT-MetaMATH-SV(Self-Verification) & 156& & TODO \\
%SFT-MetaMATH-FOBAR & 156& & TODO \\
\rowcolor{Gray} SFT‑DecompX (Ours)& xxx      &  $42.68 \pm 3.87$ \\
%\midrule
% \rowcolor{Gray} SFT‑DecompX + Curriculum (Ours)& xxx & xxx\\
%\rowcolor{Gray} SFT-DecompX + Curriculum + Original (ours) & 415 & $16.7 \pm 6.9$ (evaluating more in Node2) \\
\midrule
\multicolumn{3}{c}{\textit{\textbf{DeepSeek-R1-Distill-Qwen-1.5B SFT on Codeforces-CoTs}}} \\
\midrule
Base                 & N.A.   & $36.01 \pm 1.85$ \\
% SFT                  & xxx      & $35.37 \pm 3.74$ \\
%SFT-MetaMATH-AnsAug(Answer Augmentation) & 60& & TODO \\
%SFT-MetaMATH-Rephrasing & 60& & TODO \\
%SFT-MetaMATH-SV(Self-Verification) & 156& & TODO \\
%SFT-MetaMATH-FOBAR & 156& & TODO \\
\rowcolor{Gray} SFT‑DecompX (Ours)& xxx      &  $57.90 \pm 0.98$ \\
%\midrule
% \rowcolor{Gray} SFT‑DecompX + Curriculum (Ours)& xxx & xxx\\
\bottomrule
\end{tabular}
\end{table*}


==> datadecomposition.tex <==

\todo{need to rewrite this part}

\paragraph{Input.}
We consider a dataset \( \mathcal{D}^{(0)} = \{(x^{(0)}, y^{(0)})\} \), where each \( x^{(0)} \) is a complex math problem and \( y^{(0)} \) is its final answer. A teacher model \( \mathcal{T} \) (e.g., GPT-4o) is used to generate multi-step solutions via chain-of-thought prompting.

\paragraph{Output.}
The objective is to construct a decomposed dataset \( \mathcal{D}' = \{(x^{(d)}, y^{(d)})\} \), where each subproblem \( x^{(d)} \) represents a localized reasoning task at recursion depth \( d \), paired with a verified subanswer \( y^{(d)} \).

\paragraph{Recursive Decomposition.}
Given an initial problem \( x^{(0)} \), we apply the teacher model to generate a reasoning trace:
\[
x^{(0)} \mapsto \text{cot}^{(0)} = [s_1, s_2, \dots, s_T].
\]
Each intermediate step \( s_k \in \text{cot}^{(0)} \) is treated as a semantic anchor for a new subproblem \( x^{(1)}_k \). For each such subproblem, the model generates a corresponding answer \( \hat{y}^{(1)}_k \) and a refined reasoning chain \( \text{cot}^{(1)}_k \). The same decomposition process is recursively applied to each accepted subproblem:
\[
(x^{(d-1)}, y^{(d-1)}) \mapsto \{(x^{(d)}, y^{(d)})\}.
\]

\paragraph{Recurrsive Representation.}
The full decomposition yields a rooted tree \( \mathcal{T} \), where each node is a verified tuple \( (x^{(d)}, y^{(d)}) \) and each edge denotes a dependency relation between reasoning steps. The structure reflects the recursive trace of the original solution while abstracting intermediate mathematical operations as separate tasks.

\paragraph{Verification.}
Each candidate subanswer \( \hat{y}^{(d)} \) is verified through model-based consistency checking. %Specifically, we prompt the teacher model with a direct solution query for \( x^{(d)} \) in the following form:
%\begin{quote}
%\small
%``Solve this question step by step.\newline
%\texttt{\{x^{(d)}\}}\newline
%Provide only the final numerical answer (e.g., 7.5, 4, 5/324), no explanation.''
%\end{quote}
The subanswer is accepted if the re-generated final answer matches \( \hat{y}^{(d)} \). This self-verification process filters out invalid generations and ensures logical consistency across recursive steps. Subproblems failing verification are discarded or regenerated with a modified prompt. For efficiency, verification is retried up to a fixed number of attempts.



==> math_small_table.tex <==
\begin{table*}[t!]
\centering
\caption{Comparison of testing accuracy to LLMs on the AIME 2025 benchmark. \# data refers to the number of examples used for fine-tuning. \footnotesize $^\ddag$We evaluate based on the checkpoint released at https://huggingface.co/simplescaling/s1-32B without budget forcing. }
\label{tab:perf_aime2025}
\begin{tabular}{lcc}
\toprule
\bf Model & \bf \makecell{\# data} & \bf \makecell{AIME2025} \\
%Flash Think.         &            &      \\
\midrule
\multicolumn{3}{c}{\textit{\textbf{DeepSeek-R1-Distill-Qwen-1.5B SFT on MATH}}} \\
\midrule
Base                 & N.A.   & $23.33 \pm 7.85$ \\
% SFT                  & xxx      & $35.37 \pm 3.74$ \\
%SFT-MetaMATH-AnsAug(Answer Augmentation) & 60& & TODO \\
%SFT-MetaMATH-Rephrasing & 60& & TODO \\
%SFT-MetaMATH-SV(Self-Verification) & 156& & TODO \\
%SFT-MetaMATH-FOBAR & 156& & TODO \\
\rowcolor{Gray} SFT‑DecompX (Ours)& 4500      &  $30.00 \pm 8.51
$ \\
%\midrule
%\rowcolor{Gray} SFT‑DecompX + Curriculum (Ours)& xxx & xxx\\
\bottomrule
\end{tabular}
\end{table*}

==> math_tag_table.tex <==

\begin{table*}[htbp]
\centering
\caption{\textbf{Summary of Cluster Tags}. Sample count represents the number of questions associated with each cluster tag. Keywords are derived from the tags within each cluster.}
\tiny
\begin{tabular}{>{\raggedright}p{3.5cm} l p{9cm}}
\toprule
Domain & \#questions & Keywords \\
\midrule
Counting \& Probability & 32 & Counting \& Probability \\
Counting Principle & 15 & Counting Principle, Counting Principles, Fundamental Counting Principle, Fundamental Principle of Counting \\
Combination Calculation & 11 & Combination Calculation, Combination Formula, Combinations, Combinations Calculation, Combinations Formula, Counting Combinations \\
Linear Equation Evaluation & 9 & Linear Equation Evaluation, Linear Equation Solving, Linear Expression Evaluation, Solving Linear Equations \\
Combinatorial Counting & 9 & Combinatorial Counting, Combinatorics, Counting, Counting Subsets \\
Binomial Coefficient & 8 & Binomial Coefficient, Binomial Coefficient Calculation, Binomial Coefficient Simplification, Binomial Coefficients, Binomial Coefficients Calculation, Binomial Expansion, Binomial Theorem \\
Factorial Calculation & 8 & Factorial Calculation, Factorial Division, Factorial Multiplication, Factorial Simplification \\
Addition & 7 & Addition, Addition of integers, Arithmetic Addition, Integer Addition \\
Division Property of Equality & 7 & Division Property of Equality \\
Exponentiation & 7 & Exponentiation, Exponentiation Principle \\
Division Simplification & 6 & Division Simplification, Fraction Simplification \\
Summation & 5 & Summation, Summation of a Sequence \\
Arithmetic Operations & 5 & Arithmetic Operations, Multiplication, Multiplication of Integers \\
Arithmetic with Fractions & 5 & Arithmetic with Fractions, Division of Fractions, Fraction Division, Fraction Multiplication, Fraction Subtraction, Subtracting Fractions with Common Denominator, Subtracting Fractions with Common Denominators \\
Circular Permutations & 5 & Circular Permutations, Cyclic Permutations, Permutations \\
Arithmetic Sequence & 4 & Arithmetic Sequence, Arithmetic Sequence Formula, Arithmetic Sequence Identification, Arithmetic Sequence Sum, Arithmetic Sequence Sum Formula, Arithmetic Sequences \\
Substitution & 4 & Substitution, Substitution Method, Variable Substitution \\
Independent Events Probability Calculation & 4 & Independent Events Probability Calculation, Independent Probability, Probability Calculation, Probability of Independent Events \\
Arithmetic Series Formula & 4 & Arithmetic Series Formula, Arithmetic Series Sum Formula, Arithmetic Series Summation, Arithmetic Sum Calculation, Summation of Arithmetic Series \\
Place Value & 4 & Place Value \\
Equation Simplification & 3 & Equation Simplification, Linear Equation Simplification \\
Counting Integers & 3 & Counting Integers, Counting Integers in a Range \\
Isolating Variables & 3 & Isolating Variables, Isolating the variable \\
GCD Calculation & 3 & GCD Calculation \\
Simplifying Fractions & 3 & Simplifying Fractions \\
Subtraction & 3 & Subtraction \\
Permutations with Repetition & 3 & Permutations with Repetition, Permutations without repetition \\
Long Division & 2 & Long Division \\
Probability Distribution & 2 & Probability Distribution \\
Complementary Counting & 2 & Complementary Counting \\
Divisibility Rules & 2 & Divisibility Rules \\
Factoring by grouping & 2 & Factoring by grouping, Factorization \\
Combining Like Terms & 2 & Combining Like Terms \\
Intersection of Lines and Curves & 2 & Intersection of Lines and Curves, Line Intersection \\
Common Denominator Calculation & 2 & Common Denominator Calculation, Common Denominator Conversion \\
Complement Rule & 2 & Complement Rule, Complement Rule in Probability \\
Complementary Probability & 2 & Complementary Probability \\
Probability Addition Rule & 2 & Probability Addition Rule, Total Probability Rule \\
Permutation Calculation & 2 & Permutation Calculation, Permutations and Combinations \\
Addition and Subtraction Properties of Equality & 2 & Addition and Subtraction Properties of Equality \\
Factoring Common Factor & 2 & Factoring Common Factor, Factoring Out Common Factors, Finding Factors \\
Long Multiplication & 2 & Long Multiplication, Multiplication of Large Numbers \\
Counting Even Numbers & 2 & Counting Even Numbers, Counting Odd Numbers, Identifying Even Numbers \\
Independent Probability Multiplication & 2 & Independent Probability Multiplication, Multiplication Rule for Independent Events \\
Percentage Calculation & 2 & Percentage Calculation, Percentage Conversion, Percentage to Decimal Conversion \\
Parity & 2 & Parity \\
Counting Leap Years & 1 & Counting Leap Years, Leap Year Calculation \\
Minimum Value Calculation & 1 & Minimum Value Calculation \\
Pigeonhole Principle & 1 & Pigeonhole Principle \\
Range Calculation & 1 & Range Calculation \\
Range of Sums for Dice Rolls & 1 & Range of Sums for Dice Rolls \\
Uniform Probability Distribution & 1 & Uniform Probability Distribution \\
Distributive Property & 1 & Distributive Property \\
Factoring Quadratic Expressions & 1 & Factoring Quadratic Expressions \\
Multiples Identification & 1 & Multiples Identification \\
Simultaneous Equations & 1 & Simultaneous Equations \\
Distance Comparison & 1 & Distance Comparison \\
Absolute Value Simplification & 1 & Absolute Value Simplification \\
Area Calculation & 1 & Area Calculation, Area Calculation of a Square, Area of a Square Calculation, Area of a Triangle Calculation \\
Area of a Right Triangle & 1 & Area of a Right Triangle, Area of a Triangle \\
Area of a Square & 1 & Area of a Square \\
Area of a Triangle Using Determinants & 1 & Area of a Triangle Using Determinants \\
Distance Formula & 1 & Distance Formula \\
Graphing Linear Inequalities & 1 & Graphing Linear Inequalities, Linear Inequality Graphing \\
Isosceles Right Triangle & 1 & Isosceles Right Triangle \\
Shoelace Theorem & 1 & Shoelace Theorem \\
Cardinality & 1 & Cardinality \\
Counting Non-Empty Subsets & 1 & Counting Non-Empty Subsets, Counting Subsets of a Set \\
Power Set Calculation & 1 & Power Set Calculation \\
Set Notation & 1 & Set Notation \\
Subset Definition & 1 & Subset Definition \\
Subset Identification & 1 & Subset Identification, Subset Selection \\
Equivalent Fractions & 1 & Equivalent Fractions \\
Factorial Decomposition & 1 & Factorial Decomposition \\
Binomial Coefficient Parity & 1 & Binomial Coefficient Parity, Parity of Binomial Coefficients \\
Pascal's Triangle & 1 & Pascal's Triangle, Pascal's Triangle Construction \\
Classifying Integers & 1 & Classifying Integers, Identifying Positive Integers \\
Identifying Negative Numbers & 1 & Identifying Negative Numbers \\
Integer Pair Sign Analysis & 1 & Integer Pair Sign Analysis \\
Sign of a Product & 1 & Sign of a Product \\
Counting Intersections & 1 & Counting Intersections, Counting intersections \\
Enumeration & 1 & Enumeration \\
Intersection of Sets & 1 & Intersection of Sets \\
Set Union & 1 & Set Union \\
Decimal Multiplication & 1 & Decimal Multiplication \\
Percentage to Fraction Conversion & 1 & Percentage to Fraction Conversion \\
Sliding Window Technique & 1 & Sliding Window Technique \\
Counting Grid Positions & 1 & Counting Grid Positions, Counting Rectangles in a Grid, Counting Subsets in a Grid \\
Counting Rows and Columns & 1 & Counting Rows and Columns \\
Counting Squares & 1 & Counting Squares \\
Counting Subgrids & 1 & Counting Subgrids \\
Indexing in Arrays & 1 & Indexing in Arrays \\
Digit Sum Calculation & 1 & Digit Sum Calculation \\
Equation Rearrangement & 1 & Equation Rearrangement \\
Modular Arithmetic & 1 & Modular Arithmetic \\
Pairing Numbers for a Fixed Sum & 1 & Pairing Numbers for a Fixed Sum \\
Summation of Consecutive Integers & 1 & Summation of Consecutive Integers \\
Symmetry in Polygons & 1 & Symmetry in Polygons \\
System of Equations & 1 & System of Equations, System of Linear Equations \\
Trial and Error & 1 & Trial and Error \\
Cross Multiplication & 1 & Cross Multiplication, Cross-Multiplication \\
Final Answer Verification & 1 & Final Answer Verification \\
Identifying Given Information & 1 & Identifying Given Information \\
Proportion Solving & 1 & Proportion Solving \\
Variable Definition & 1 & Variable Definition \\
Palindrome Construction & 1 & Palindrome Construction, Palindrome Identification \\
Case Analysis & 1 & Case Analysis \\
Casework & 1 & Casework \\
Multiplication Principle & 1 & Multiplication Principle \\
Boxing the final answer & 1 & Boxing the final answer \\
Division of Constants & 1 & Division of Constants \\
Equation Balancing & 1 & Equation Balancing \\
Initial Value Problem & 1 & Initial Value Problem \\
Recurrence Relation & 1 & Recurrence Relation, Recurrence Relations \\
Counting Frequency & 1 & Counting Frequency \\
Digit Frequency Analysis & 1 & Digit Frequency Analysis \\
Identifying Repeating Digits in Numbers & 1 & Identifying Repeating Digits in Numbers, Repetition of Digits \\
Mode Calculation & 1 & Mode Calculation \\
Initial Value Identification & 1 & Initial Value Identification \\
Parity Constraint & 1 & Parity Constraint \\
Parity of Digits & 1 & Parity of Digits \\
Digit Placement & 1 & Digit Placement \\
Permutations with restrictions & 1 & Permutations with restrictions \\
Symmetry in Probability & 1 & Symmetry in Probability \\
Counting Exclusion & 1 & Counting Exclusion \\
Range Exclusion & 1 & Range Exclusion \\
Multiplication of Powers of 10 & 1 & Multiplication of Powers of 10 \\
\midrule
\textbf{Total} & 247 & \\
\bottomrule
\end{tabular}
\label{tab:tag_usage}
\end{table*}
\newpage


==> table2.tex <==
\begin{table}[htbp]
\centering
\caption{We evaluate \ours{} (some entries are unknown (N.A.), see \autoref{sec:results}). Other results are from the respective reports~\citep{qwen2024qwen25technicalreport,qwq-32b-preview,o1,r1,bespoke_stratos,sky_t1}. \# ex. = number examples used for reasoning finetuning.}
\begin{tabular}{lccc}
\toprule
Model & \makecell{\# ex.} & \makecell{AIME2024} & \makecell{AIME2025} \\
%Flash Think.         &            &      \\
\midrule
\multicolumn{4}{c}{\textbf{Open-Source Models}} \\
\midrule
Qwen2.5-72B-Instruct  & N.A.     & 43.3  & 15.0 \\
s1(ours)                    & 1000     & 46.7 & 13.3 \\
\midrule
\multicolumn{4}{c}{\textbf{Close-Source Models}} \\
\midrule
GPT-4o               & N.A.     & 9.3 & 7.6 \\
\midrule
\multicolumn{4}{c}{\textbf{Qwen3-4B-Base SFT on AIME2024}} \\
\midrule
Base                 & N.A. &  $3.33 \pm 3.33$    & $10.0 \pm 5.57$ \\
SFT                  & 30      & $6.67 \pm 4.63$  & $3.33 \pm 3.33$ \\
SFT-MetaMATH-Augmentation & 432& TODO & TODO \\
%SFT-MetaMATH-AnsAug(Answer Augmentation) & 60& & TODO \\
%SFT-MetaMATH-Rephrasing & 60& & TODO \\
%SFT-MetaMATH-SV(Self-Verification) & 156& & TODO \\
%SFT-MetaMATH-FOBAR & 156& & TODO \\
SFT‑decomposed (ours)& 385      & $6.67 \pm 4.63$ & $13.33 \pm 6.31$ \\
\midrule
SFT‑decomposed‑curriculum (ours)& 385 & $10.0 \pm 5.57$ & $16.67 \pm 6.92$ \\
SFT-decomposed-curriculum+Original (ours) & 415 & (TODO) & (TODO) \\
\bottomrule
\label{tab:perf_aime2025}
\end{tabular}
\end{table}

==> table3.tex <==
\begin{table}[t]
    \centering
    % \sffamily
    \tiny
    \begin{tabular}{p{0.48\linewidth}|p{0.48\linewidth}}
    \toprule 
       \cellcolor[HTML]{dfaea3} \textbf{Bad data} & \cellcolor[HTML]{cce2c3}  \textbf{Good data} \\
    \midrule
       \colorbox[HTML]{a9c5f6}{English} \textbf{\textcolor[HTML]{ce9178}{Mismatched Answer}}
       \newline
       \colorbox[HTML]{dfaea3}{\textbf{Score: -0.714698731899261}}
       \newline

\textbf{Problem:} Simplify $\frac{3^4+3^2}{3^3-3}$.Express your answer as a common fraction.\newline
\textbf{Solution:} The common factor of 3 in the numerator and the common factor of 3 in the denominator will cancel: $\frac{3^4+3^2}{3^3-3}=\frac{3(3^3+3^1)}{3(3^2-1)}=\frac{3^3+3^1}{3^2-1}$. Now the numerator is $3^3+3=27+3=30$, and the denominator is $3^2-1=9-1=8$.  Therefore, the fraction simplifies to $\dfrac{30}{8}=\boxed{\dfrac{15}{4}}$.

  & \colorbox[HTML]{a9c5f6}{Lower Difficulty Generated Data} \colorbox[HTML]{cce2c3}{\textbf{Difficulty Score:4.0}} \newline

[instruction] Given your background as a doctor, please provide your insight in addressing the medical questions based on the patient's account. \newline

[input] A 52-year-old man presents to his primary care physician for generalized pain. … Which of the following is associated with this patient's condition?. A. Hearing loss B. Bence Jones proteins C. Hypercalcemia D. Obstructive jaundice \newline

[output] Hearing loss. Choosing option A, hearing loss, may seem counterintuitive given the patient‘s primary complaint of generalized pain. However, the notable aspect of the case is the elevated alkaline phosphatase (ALP) level while other liver function tests (AST, ALT) and lipase are normal, suggesting the source of the ALP is likely not the liver or pancreas. The combination of bone pain and elevated ALP can be suggestive of Paget’s disease of bone, which is associated with osteoskeletal changes leading to hearing loss due to auditory nerve compression or bony encroachment of the inner ear structures. \newline

 \\ \hline
 \colorbox[HTML]{a9c5f6}{Chinese}  \textbf{\textcolor[HTML]{ce9178}{Incomplete Answer}}\newline
\colorbox[HTML]{dfaea3}{\textbf{Score: -0.42757144570350647}} \newline
\begin{CJK}{UTF8}{gbsn}
[instruction] 
 \colorbox[HTML]{a9c5f6}{Chinese}  \colorbox[HTML]{cce2c3}{\textbf{Score: 0.23900631070137024}} \newline
[instruction] 

\end{CJK} \\ \hline
 \colorbox[HTML]{a9c5f6}{Spanish} Mixed Languages \newline
 
\colorbox[HTML]{dfaea3}{\textbf{Score: -0.6730865836143494}} \newline
[instruction] 

[output] 
& 
\colorbox[HTML]{a9c5f6}{Higher Difficulty Generated Data} 
 \colorbox[HTML]{cce2c3}{\textbf{Difficulty Score: 18.0}}
 
\textbf{Problem:} Simplify the expression $\frac{3^3 + 3}{3^2 - 1}$. \newline
\textbf{Solution:} Compute the powers$3^3 = 27, 3^2 = 9$. Substitute into the expression:
$\frac{27 + 3}{9 - 1}$. Perform addition and subtraction$\frac{30}{8}$. Simplify the fraction$\frac{30}{8} = \frac{15}{4}$. Final Answer is $\boxed{\frac{15}{4}}$. 

\textbf{Problem:} What is the greatest common divisor (GCD) of the numbers 30 and 8? \newline
\textbf{Solution:} To find the greatest common divisor (GCD) of 30 and 8, we need to identify the largest number that divides both 30 and 8 without leaving a remainder.\n\n1. List the factors of 30:\n   - 1, 2, 3, 5, 6, 10, 15, 30\n\n2. List the factors of 8:\n   - 1, 2, 4, 8\n\n3. Identify the common factors of 30 and 8:\n   - The common factors are 1 and 2.\n\n4. The greatest of these common factors is 2.

\textbf{Problem:} What is the value of $3^3$? \newline
\textbf{Solution:} To solve for $3^3$, we need to perform exponentiation, which involves multiplying the base number by itself a certain number of times. In this case, the base number is 3 and the exponent is 3. This means we multiply 3 by itself three times:\n\n1. First, multiply 3 by 3: $3 \times 3 = 9$. 2. Next, take the result and multiply by 3 again: $9 \times 3 = 27$. Therefore, the value of $3^3$ is 27.
\vspace{1em}
\\
     \bottomrule
    \end{tabular}
    \caption{Caption TBD}
    \label{tab:training_examples}
\end{table}


\begin{table}[t]
    \centering
    \tiny
    \begin{tabular}{p{0.48\linewidth}|p{0.48\linewidth}}
    \toprule 
       \cellcolor[HTML]{dfaea3} \textbf{Bad data} & \cellcolor[HTML]{cce2c3}  \textbf{Good data} \\
    \midrule
       \multirow{3}{=}{%
       \colorbox[HTML]{a9c5f6}{English} \textbf{\textcolor[HTML]{ce9178}{Mismatched Answer}}
       \newline
       \colorbox[HTML]{dfaea3}{\textbf{Score: -0.714698731899261}}
       \newline

\textbf{Problem:} Simplify $\frac{3^4+3^2}{3^3-3}$.Express your answer as a common fraction.\newline
\textbf{Solution:} The common factor of 3 in the numerator and the common factor of 3 in the denominator will cancel: $\frac{3^4+3^2}{3^3-3}=\frac{3(3^3+3^1)}{3(3^2-1)}=\frac{3^3+3^1}{3^2-1}$. Now the numerator is $3^3+3=27+3=30$, and the denominator is $3^2-1=9-1=8$.  Therefore, the fraction simplifies to $\dfrac{30}{8}=\boxed{\dfrac{15}{4}}$.} 
& 
\colorbox[HTML]{a9c5f6}{Lower Difficulty Generated Data} \colorbox[HTML]{cce2c3}{\textbf{Difficulty Score:4.0}} \newline

[instruction] Given your background as a doctor, please provide your insight in addressing the medical questions based on the patient's account. \newline

[input] A 52-year-old man presents to his primary care physician for generalized pain. … Which of the following is associated with this patient's condition?. A. Hearing loss B. Bence Jones proteins C. Hypercalcemia D. Obstructive jaundice \newline

[output] Hearing loss. Choosing option A, hearing loss, may seem counterintuitive given the patient‘s primary complaint of generalized pain. However, the notable aspect of the case is the elevated alkaline phosphatase (ALP) level while other liver function tests (AST, ALT) and lipase are normal, suggesting the source of the ALP is likely not the liver or pancreas. The combination of bone pain and elevated ALP can be suggestive of Paget’s disease of bone, which is associated with osteoskeletal changes leading to hearing loss due to auditory nerve compression or bony encroachment of the inner ear structures. 
\\ \cline{2-2}
 & 
\colorbox[HTML]{a9c5f6}{Higher Difficulty Generated Data} 
 \colorbox[HTML]{cce2c3}{\textbf{Difficulty Score: 18.0}}
 
\textbf{Problem:} Simplify the expression $\frac{3^3 + 3}{3^2 - 1}$. \newline
\textbf{Solution:} Compute the powers $3^3 = 27$, $3^2 = 9$. Substitute into the expression:
$\frac{27 + 3}{9 - 1}$. Perform addition and subtraction: $\frac{30}{8}$. Simplify the fraction: $\frac{30}{8} = \frac{15}{4}$. Final Answer is $\boxed{\frac{15}{4}}$. 

\textbf{Problem:} What is the greatest common divisor (GCD) of the numbers 30 and 8? \newline
\textbf{Solution:} To find the greatest common divisor (GCD) of 30 and 8, we need to identify the largest number that divides both 30 and 8 without leaving a remainder. The GCD is 2.

\textbf{Problem:} What is the value of $3^3$? \newline
\textbf{Solution:} $3^3 = 3 \times 3 \times 3 = 27$.

\textbf{Follow-up:} How would this solution change if the denominator was $3^2 + 1$ instead of $3^2 - 1$? \newline
\textbf{Answer:} If the expression is $\frac{3^3 + 3}{3^2 + 1} = \frac{30}{10} = 3$.
\\
     \bottomrule
    \end{tabular}
    \caption{Caption TBD}
    \label{tab:training_examples}
\end{table}

==> table33.tex <==
\begin{table}[tbp]
    \centering
    \caption{Examples of an original data sample from MATH training set and its generated data samples.}
    \scriptsize	
    \begin{tabular}{p{0.48\linewidth}|p{0.48\linewidth}}
    \toprule 
       \cellcolor[HTML]{dfaea3} \textbf{Original Data} & \cellcolor[HTML]{cce2c3}  \textbf{Decomposed Data} \\
    \midrule
    \multirow{3}{=}{%
\newline

\textbf{Problem:} Simplify $\frac{3^4+3^2}{3^3-3}$. Express your answer as a common fraction.\newline
\textbf{Solution:} The common factor of 3 in the numerator and the denominator can be factored out: $\frac{3^4+3^2}{3^3-3}=\frac{3(3^3+3)}{3(3^2-1)}=\frac{3^3+3}{3^2-1}$. Now compute: numerator is $27+3=30$, denominator is $9-1=8$, so $\frac{30}{8} = \boxed{\frac{15}{4}}$.} 
& 
\colorbox[HTML]{a9c5f6}{Lower Difficulty Generated Data} \colorbox[HTML]{cce2c3}{\textbf{Difficulty Score: 4.0}} \newline

\textbf{Problem:} What is the value of $3^3$? \newline
\textbf{Solution:} To solve for $3^3$, we need to perform exponentiation, which involves multiplying the base number by itself a certain number of times. In this case, the base number is 3 and the exponent is 3. This means we multiply 3 by itself three times:\n\n1. First, multiply 3 by 3: $3 \times 3 = 9$. 2. Next, take the result and multiply by 3 again: $9 \times 3 = 27$. Therefore, the value of $3^3$ is 27. \newline
\textbf{Tag:} Exponentiation

\\ \cline{2-2}
& 
\colorbox[HTML]{a9c5f6}{Medium Difficulty Generated Data} \colorbox[HTML]{cce2c3}{\textbf{Difficulty Score: 10.0}} \newline

\textbf{Problem:} What is the greatest common divisor (GCD) of the numbers 30 and 8? \newline
\textbf{Solution:} To find the greatest common divisor (GCD) of 30 and 8, we need to identify the largest number that divides both 30 and 8 without leaving a remainder.\n\n1. List the factors of 30:\n   - 1, 2, 3, 5, 6, 10, 15, 30\n\n2. List the factors of 8:\n   - 1, 2, 4, 8\n\n3. Identify the common factors of 30 and 8:\n   - The common factors are 1 and 2.\n\n4. The greatest of these common factors is 2.\newline
\textbf{Tag:} GCD Calculation\\
\\ \cline{2-2}
& 
\colorbox[HTML]{a9c5f6}{Higher Difficulty Generated Data} \colorbox[HTML]{cce2c3}{\textbf{Difficulty Score: 18.0}} \newline

\textbf{Problem:} Simplify the expression $\frac{3^3 + 3}{3^2 - 1}$. \newline
\textbf{Solution:} We first compute the powers$3^3 = 27, 3^2 = 9$. Next, substitute into the expression:
$\frac{27 + 3}{9 - 1}$. Perform addition and subtraction$\frac{30}{8}$. And simplify the fraction$\frac{30}{8} = \frac{15}{4}$. Final Answer is $\boxed{\frac{15}{4}}$. \newline
\textbf{Tag:} Fraction Simplification
\\
\bottomrule
\end{tabular}
% \caption{Examples of low-quality and high-quality training data}
\label{tab:data_examples}
\end{table}

==> table4.tex <==
\begin{table}[t]
    \centering
    \tiny
    \begin{tabular}{p{0.48\linewidth}|p{0.48\linewidth}}
    \toprule 
       \cellcolor[HTML]{dfaea3} \textbf{Original Data} & \cellcolor[HTML]{cce2c3}  \textbf{Decomposed Data} \\
    \midrule
    \multirow{3}{=}{%
\newline

\textbf{Problem:} Simplify $\frac{3^4+3^2}{3^3-3}$. Express your answer as a common fraction.\newline
\textbf{Solution:} The common factor of 3 in the numerator and the denominator can be factored out: $\frac{3^4+3^2}{3^3-3}=\frac{3(3^3+3)}{3(3^2-1)}=\frac{3^3+3}{3^2-1}$. Now compute: numerator is $27+3=30$, denominator is $9-1=8$, so $\frac{30}{8} = \boxed{\frac{15}{4}}$.} 
& 
\colorbox[HTML]{a9c5f6}{Lower Difficulty Generated Data} \colorbox[HTML]{cce2c3}{\textbf{Difficulty Score: 4.0}} \newline

\textbf{Problem:} What is the value of $3^3$? \newline
\textbf{Solution:} To solve for $3^3$, we need to perform exponentiation, which involves multiplying the base number by itself a certain number of times. In this case, the base number is 3 and the exponent is 3. This means we multiply 3 by itself three times:\n\n1. First, multiply 3 by 3: $3 \times 3 = 9$. 2. Next, take the result and multiply by 3 again: $9 \times 3 = 27$. Therefore, the value of $3^3$ is 27. \newline
\textbf{Tag:} Exponentiation

\\ \cline{2-2}
& 
\colorbox[HTML]{a9c5f6}{Midie Difficulty Generated Data} \colorbox[HTML]{cce2c3}{\textbf{Difficulty Score: 10.0}} \newline

\textbf{Problem:} What is the greatest common divisor (GCD) of the numbers 30 and 8? \newline
\textbf{Solution:} To find the greatest common divisor (GCD) of 30 and 8, we need to identify the largest number that divides both 30 and 8 without leaving a remainder.\n\n1. List the factors of 30:\n   - 1, 2, 3, 5, 6, 10, 15, 30\n\n2. List the factors of 8:\n   - 1, 2, 4, 8\n\n3. Identify the common factors of 30 and 8:\n   - The common factors are 1 and 2.\n\n4. The greatest of these common factors is 2.\newline
\textbf{Tag:} GCD Calculation
\\ \cline{2-2}
& 
\colorbox[HTML]{a9c5f6}{High Difficulty Generated Data} \colorbox[HTML]{cce2c3}{\textbf{Difficulty Score: 18.0}} \newline

\textbf{Problem:} Simplify the expression $\frac{3^3 + 3}{3^2 - 1}$. \newline
\textbf{Solution:} Compute the powers$3^3 = 27, 3^2 = 9$. Substitute into the expression:
$\frac{27 + 3}{9 - 1}$. Perform addition and subtraction$\frac{30}{8}$. Simplify the fraction$\frac{30}{8} = \frac{15}{4}$. Final Answer is $\boxed{\frac{15}{4}}$. \newline
\textbf{Tag:} Fraction Simplification
\\
\bottomrule
\end{tabular}
\caption{Examples of low-quality and high-quality training data}
\label{tab:training_examples}
\end{table}

